Transfer Generative Adversarial Networks (T-GAN)-based Terahertz Channel Modeling

Terahertz (THz) communications are envisioned as a promising technology for 6G and beyond wireless systems, providing ultra-broad bandwidth and thus Terabit-per-second (Tbps) data rates. However, as foundation of designing THz communications, channel modeling and characterization are fundamental to scrutinize the potential of the new spectrum. Relied on physical measurements, traditional statistical channel modeling methods suffer from the problem of low accuracy with the assumed certain distributions and empirical parameters. Moreover, it is time-consuming and expensive to acquire extensive channel measurement in the THz band. In this paper, a transfer generative adversarial network (T-GAN) based modeling method is proposed in the THz band, which exploits the advantage of GAN in modeling the complex distribution, and the benefit of transfer learning in transferring the knowledge from a source task to improve generalization about the target task with limited training data. Specifically, to start with, the proposed GAN is pre-trained using the simulated dataset, generated by the standard channel model from 3rd generation partnerships project (3GPP). Furthermore, by transferring the knowledge and fine-tuning the pre-trained GAN, the T-GAN is developed by using the THz measured dataset with a small amount. Experimental results reveal that the distribution of PDPs generated by the proposed T-GAN method shows good agreement with measurement. Moreover, T-GAN achieves good performance in channel modeling, with 9 dB improved root-mean-square error (RMSE) and higher Structure Similarity Index Measure (SSIM), compared with traditional 3GPP method.

==> system.tex <==
\section{Problem Formulation}\label{sec_system}
% In this paper, I consider modeling THz SISO channel in an indoor corridor scenario. To model the channel in this scenario, the measurement campaign is conducted in~\cite{yuanbo_icc} with a frequency-domain Vector Network Analyzer (VNA)-based channel sounder. The positions of transmitter and receiver are carefully chosen to characterize the propagation environment in the corridor. Based on the measurement results, 
the channel impulse response (CIR) can be obtained, which can be represented as 
\begin{equation}
    h(\tau) =\sum_{l=0}^{L-1}\alpha_le^{j\phi_l}\delta(\tau-\tau_l),
\end{equation}
where $\tau$ refers to the propagation delay, $\tau_l$ denotes the delay$L$ of the $l$-th multipath, $L$ denotes the number of multi-paths, $\alpha_l$ refers to the path gain and $\phi_l$ represents the phase of the corresponding multi-path. To characterize the channel, power delay profile (PDP) is an important feature, which indicates the dispersion of power over the time delay. It represents the received power with respect to the time of delay in a multi-path channel, which can be extracted from the CIR by
\begin{equation}
    P(\tau) = |h(\tau)|^2.
\end{equation}
Then, the channel modeling problem is to model the distribution of PDP, such that the statistical property of generated distribution of PDP can match the distribution of measurement.









% the 3GPP SISO channel model implemented by Quadriga is considered, while the important statistics of channel are collected from realistic THz measurement campaign~\cite{yuanbo_icc}. 

% I denote the distribution of channel generated by 3GPP model by $P_r$, and the channel samples from the distribution are considered as real channel. The channel modeling problem is formulated as finding the approximate distribution $P_g$, that is close to the real distribution $P_r$. Then, the problem is to minimize the distribution between the two distributions, represented by
% \begin{equation}
%     W(P_r,P_g)=\inf_{\gamma\in \prod(P_r,P_g)}E_{(x,y)\sim\gamma}(\left\|x-y\right\|).
% \end{equation}
% The distance metric chosen is the Earth-Mover (EM) Distance, which can be considered as the optimal cost to transform between two distributions. 



